Augmenting NER Datasets with LLMs: Towards Automated and Refined Annotation

In the field of Natural Language Processing (NLP), Named Entity Recognition (NER) is recognized as a critical technology, employed across a wide array of applications. Traditional methodologies for annotating datasets for NER models are challenged by high costs and variations in dataset quality. This research introduces a novel hybrid annotation approach that synergizes human effort with the capabilities of Large Language Models (LLMs). This approach not only aims to ameliorate the noise inherent in manual annotations, such as omissions, thereby enhancing the performance of NER models, but also achieves this in a cost-effective manner. Additionally, by employing a label mixing strategy, it addresses the issue of class imbalance encountered in LLM-based annotations. Through an analysis across multiple datasets, this method has been consistently shown to provide superior performance compared to traditional annotation methods, even under constrained budget conditions. This study illuminates the potential of leveraging LLMs to improve dataset quality, introduces a novel technique to mitigate class imbalances, and demonstrates the feasibility of achieving high-performance NER in a cost-effective way.

==> latex/02_preliminary.tex <==
% \section{Preliminary}

% \begin{description}[leftmargin=*,itemsep=0pt,topsep=0pt]

% \item[Named Entity Recognition (NER) task:]

% The Named Entity Recognition (NER) task in Natural Language Processing involves identifying and classifying named entities in text into predefined categories such as persons, organizations, locations, etc \cite{nadeau2007survey, Li2018ASO}. 
% The primary objective of NER is to minimize inaccuracies in recognizing and categorizing these entities. This section formalizes the NER task, outlining the criteria and metrics used to evaluate the performance of NER systems, and explains the challenges in accurately identifying and classifying entities in varying contexts.


% \end{description}
